MAG-Edit: Localized Image Editing in Complex Scenarios via Mask-Based Attention-Adjusted Guidance

Recent diffusion-based image editing approaches have exhibited impressive editing capabilities in images with simple compositions. However, localized editing in complex scenarios has not been well-studied in the literature, despite its growing real-world demands. Existing mask-based inpainting methods fall short of retaining the underlying structure within the edit region. Meanwhile, mask-free attention-based methods often exhibit editing leakage and misalignment in more complex compositions. In this work, we develop MAG-Edit, a training-free, inference-stage optimization method, which enables localized image editing in complex scenarios. In particular, MAG-Edit optimizes the noise latent feature in diffusion models by maximizing two mask-based cross-attention constraints of the edit token, which in turn gradually enhances the local alignment with the desired prompt. Extensive quantitative and qualitative experiments demonstrate the effectiveness of our method in achieving both text alignment and structure preservation for localized editing within complex scenarios.

==> draft.tex <==


\section{Asymmetric noise guidance}
%
The proposed optimization process continually incorporates new token-related information into $z_t$ through gradient guidance, thereby enhancing the editing granularity.
%
After completing the updating process, we use the optimized $z_t^$ to predict the new noise $\boldsymbol{\epsilon}_t^\theta\left(z_t^\right)$ and subsequently update $z_{t-1}$ as follows:
\begin{equation}
\begin{split}
z_{t-1} &=\sqrt{\alpha_{t-1}} \left(\frac{z_t^*-\sqrt{1-\alpha_t} \boldsymbol{\epsilon}_t^\theta\left(z_t^*\right)}{\sqrt{\alpha_t}}\right)\\
&+\sqrt{1-\alpha_{t-1}-\sigma_t^2} \cdot \boldsymbol{\epsilon}_t^\theta\left(z_t^*\right) +\sigma_t z_t^*.
\label{Eq:proposed9} 
\end{split}
\end{equation}
The CA maps become larger than they were before the update, which generates new noise with a more pronounced editing effect. However, we have observed that in some cases if both noise terms $\boldsymbol{\epsilon}t^\theta$ are updated simultaneously, the intermediate alterations of these terms counterbalance each other, leading to diminished guidance for $z_{t-1}$.
%
Therefore, we employ asymmetric guidance~\cite{kwon2022diffusion} to exert stronger influences. In this approach, only the first noise term is updated, while the second noise term is predicted using the un-optimized $z_t$:
%
\begin{equation}
\begin{split}
z_{t-1} &=\sqrt{\alpha_{t-1}} \left(\frac{z_t^*-\sqrt{1-\alpha_t} \boldsymbol{\epsilon}_t^\theta\left(z_t^*\right)}{\sqrt{\alpha_t}}\right)\\
&+\sqrt{1-\alpha_{t-1}-\sigma_t^2} \cdot \boldsymbol{\epsilon}_t^\theta\left(z_t\right) +\sigma_t z_t^*.
\label{Eq:proposed10} 
\end{split}
\end{equation}
















